Provable quantum state tomography via non-convex methods

With nowadays steadily growing quantum processors, it is required to develop new quantum tomography tools that are tailored for high-dimensional systems. In this work, we describe such a computational tool, based on recent ideas from non-convex optimization. The algorithm excels in the compressed-sensing-like setting, where only a few data points are measured from a low-rank or highly-pure quantum state of a high-dimensional system. We show that the algorithm can practically be used in quantum tomography problems that are beyond the reach of convex solvers, and, moreover, is faster than other state-of-the-art non-convex approaches. Crucially, we prove that, despite being a non-convex program, under mild conditions, the algorithm is guaranteed to converge to the global minimum of the problem; thus, it constitutes a provable quantum state tomography protocol.

==> preamble2.tex <==
\usepackage{amsmath,amsfonts,amsthm,amssymb,xspace,bm,bbold, bbm}
%\usepackage{verbatim,dsfont,mathtools,algorithm,algorithmic}
\usepackage{algorithm,algorithmic}
\usepackage{booktabs}
%\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\usepackage{multirow}
\usepackage{xfrac}
%\usepackage[numbers]{natbib}
%\usepackage{wrapfig}
%\usepackage{varwidth}
%\usepackage{colortbl}
\usepackage{epstopdf}
%\usepackage{appendix}
%\usepackage{enumitem}
%\usepackage{pifont}
%\usepackage[table]{xcolor}

%\usepackage{authblk}

%%%%% THEOREM STYLE DEFINITIONS
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{fact}[theorem]{Fact}
\theoremstyle{definition}
\newtheorem{question}[theorem]{Question}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}

\newcommand{\R}{\mathbb{R}}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\eqdef}{\stackrel{\textrm{def}}{=}}
\newcommand{\tr}{{\rm Tr}}
%\DeclareMathOperator{\trace}{\textsc{Tr}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\expec}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\prob}[1]{\mathbb{P}\left[#1\right]}
\newcommand{\ip}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\abs}[1]{\left \vert #1\right \vert}
\newcommand{\norm}[1]{\left \Vert #1\right \Vert}
\newcommand{\dist}{{\rm{\textsc{Dist}}}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\cmark}{\ding{51}}%

\newcommand{\obs}{y}
\newcommand{\linmap}{\mathcal{A}}

\newcommand{\plus}[1]{{#1}^{\scalebox{0.7}{+}}}
\newcommand{\mat}[1]{\mathbf{#1}}

\newcommand{\tagterm}[2]{\underbrace{#2}_{#1}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\X}{X}
\newcommand{\Y}{Y}
\newcommand{\U}{U}
\newcommand{\V}{V}
\newcommand{\E}{\mathcal{E}}
\newcommand{\gradf}{\nabla f}
\newcommand{\Xo}{X^\star}
\newcommand{\Uo}{U^\star}
\newcommand{\weta}{\widetilde{\eta}}
\newcommand{\Rus}{R_U^\star}
\newcommand{\Uw}{\widetilde{U}}
\newcommand{\QDelta}{•}
